Quantitatively Measuring and Contrastively Exploring Heterogeneity for Domain Generalization

Domain generalization (DG) is a prevalent problem in real-world applications, which aims to train well-generalized models for unseen target domains by utilizing several source domains. Since domain labels, i.e., which domain each data point is sampled from, naturally exist, most DG algorithms treat them as a kind of supervision information to improve the generalization performance. However, the original domain labels may not be the optimal supervision signal due to the lack of domain heterogeneity, i.e., the diversity among domains. For example, a sample in one domain may be closer to another domain, its original label thus can be the noise to disturb the generalization learning. Although some methods try to solve it by re-dividing domains and applying the newly generated dividing pattern, the pattern they choose may not be the most heterogeneous due to the lack of the metric for heterogeneity. In this paper, we point out that domain heterogeneity mainly lies in variant features under the invariant learning framework. With contrastive learning, we propose a learning potential-guided metric for domain heterogeneity by promoting learning variant features. Then we notice the differences between seeking variance-based heterogeneity and training invariance-based generalizable model. We thus propose a novel method called Heterogeneity-based Two-stage Contrastive Learning (HTCL) for the DG task. In the first stage, we generate the most heterogeneous dividing pattern with our contrastive metric. In the second stage, we employ an invariance-aimed contrastive learning by re-building pairs with the stable relation hinted by domains and classes, which better utilizes generated domain labels for generalization learning. Extensive experiments show HTCL better digs heterogeneity and yields great generalization performance.

==> parts/anotherabs.tex <==
\begin{abstract}
Domain generalization (DG) is a commonly encountered issue in real-world applications. Its objective is to train models that can generalize well to unseen target domains by utilizing multiple source domains. In most DG algorithms, domain labels, which indicate the domain from which each data point is sampled, are treated as a form of supervision to enhance generalization performance. However, using the original domain labels as the supervision signal may not be optimal due to a lack of diversity among domains, known as domain heterogeneity. This lack of heterogeneity can lead to the original labels being noisy and disrupting the generalization learning process. Some methods attempt to address this by re-dividing the domains and applying a new dividing pattern. However, the chosen pattern may not capture the maximum heterogeneity since there is no metric available to quantify it accurately. In this paper, we propose that domain heterogeneity primarily lies in variant features within the invariant learning framework. We introduce a novel approach, called Heterogeneity-based Two-stage Contrastive Learning (HTCL), which utilizes contrastive learning to guide the metric for domain heterogeneity. By promoting the learning of variant features, we develop a metric that captures models' learning potential for data heterogeneity. We also emphasize the distinction between seeking variance-based heterogeneity and training an invariance-based generalizable model. In the first stage of HTCL, we generate the most heterogeneous dividing pattern using our contrastive metric. In the second stage, we employ contrastive learning focused on invariance by constructing pairs based on the stable relationships indicated by domains and classes. This approach effectively utilizes the generated domain labels for generalization learning. Extensive experiments demonstrate that HTCL successfully uncovers heterogeneity and achieves remarkable generalization performance.
\end{abstract}
